Fusion of Range and Stereo Data for High-Resolution Scene-Modeling

This paper addresses the problem of range-stereo fusion, for the construction of high-resolution depth maps. In particular, we combine low-resolution depth data with high-resolution stereo data, in a maximum a posteriori (MAP) formulation. Unlike existing schemes that build on MRF optimizers, we infer the disparity map from a series of local energy minimization problems that are solved hierarchically, by growing sparse initial disparities obtained from the depth data. The accuracy of the method is not compromised, owing to three properties of the data-term in the energy function. Firstly, it incorporates a new correlation function that is capable of providing refined correlations and disparities, via subpixel correction. Secondly, the correlation scores rely on an adaptive cost aggregation step, based on the depth data. Thirdly, the stereo and depth likelihoods are adaptively fused, based on the scene texture and camera geometry. These properties lead to a more selective growing process which, unlike previous seed-growing methods, avoids the tendency to propagate incorrect disparities. The proposed method gives rise to an intrinsically efficient algorithm, which runs at 3FPS on 2.0MP images on a standard desktop computer. The strong performance of the new method is established both by quantitative comparisons with state-of-the-art methods, and by qualitative comparisons using real depth-stereo data-sets.

==> proof_of_proposition.tex <==
\begin{proof}
Let us a consider a rational function of the form (16) (EMCC function), that is
\begin{equation}\label{eq:function}
f(t) = \frac{A(t)}{B(t)},
\end{equation}
where $A(t)=\alpha_0 + \alpha_1t+\alpha_2t^2$ and $B(t)=\beta_0 + \beta_1t+\beta_2t^2$, with $B(t)$ being non degenerate. The continuous function $f(t)$ is differentiable and $f'(t)$ is also a rational function
\begin{equation}\label{eq:derivative}
f'(t) = \frac{C(t)}{B(t)^2}
\end{equation}
where
\begin{equation}\label{eq:derivative_numerator}
C(t)= c_o+c_1t+c_2t^2
\end{equation}
with
%\begin{equation}\label{eq:numerator_values}
%c_0\!=\!\alpha_1\beta_0-\beta_1\alpha_0, ~~ c_1\!=\!2(\alpha_2\beta_0-\beta_2\alpha_0),  ~~  c_2\!=\!\alpha_2\beta_1-\beta_2\alpha_1.
%\end{equation}
\begin{eqnarray}\label{eq:numerator_values}
c_0&=&\alpha_1\beta_0-\beta_1\alpha_0 \nonumber\\
c_1&=&2(\alpha_2\beta_0-\beta_2\alpha_0) \\ 
c_2&=&\alpha_2\beta_1-\beta_2\alpha_1.\nonumber
\end{eqnarray}
Since $B(t)\neq0$, $f(t)$ attains its extrema at the real roots of $C(t)$.
Let $\Delta>0$ and $t_0$, $t_1$ be the discriminant and the solutions of $C(t)=0$, respectively. Then, we can write that
\begin{equation}\label{eq:root1}
2c_2t_0+c_1 = \sqrt{\Delta}
\end{equation}
and
\begin{equation}\label{eq:root2}
2c_2t_1+c_1 = -\sqrt{\Delta}
\end{equation}
The kind of extrema can be found through the sign of the values $f''(t_0)$ and $f''(t_1)$. For the former, we obtain that
\begin{equation}\label{eq:second_derivative1}
f''(t_0) = \frac{(2c_2t_0+c_1)B(t_0)^2-2B(t_0)B'(t_0)C(t_0)}{B(t_0)^4}.
\end{equation}
From (\ref{eq:root1}), (\ref{eq:root2}) and $C(t_0)=0$, the above form is simplified to
\begin{equation}\label{eq:second_derivative1_simplified}
f''(t_0) = \frac{\sqrt{\Delta}}{B(t_0)^2}.
\end{equation}
Likewise, we obtain that
\begin{equation} \label{eq:second_derivative2}
f''(t_1) = \frac{-\sqrt{\Delta}}{B(t_1)^2}.
\end{equation}
This means that $f''(t_0)<0$ and $f''(t_1)>0$, i.e., $f(t)$ attains at most one maximum at $t_0$ and one minimum at $t_1$. The value of the maximizer, when it exists, can be extracted by using (\ref{eq:numerator_values}), (\ref{eq:root1}) and $\Delta = c_1^2-4c_0c_2$. The identification of (\ref{eq:function}) with the EMCC function (16), easily provides its maximizer. This concludes the proof.
\end{proof}


==> proposed_algorithm_R2.tex <==
As mentioned above, the initial disparity map contains noisy and biased data. Therefore, our algorithm propagates the disparity messages starting from reliable points with low energy value, \emph{without considering that their disparities reflect true matches}. If we recall the example of Fig.~\ref{fig:mrf_wta_ours}(c), this means that we exploit $d_2^0$ to restrict the disparity range of $d_3$, but once a disparity value is assigned to $d_3$, we consider $d_2$ as a node with unknown disparity. Moreover, our algorithm makes use of the subpixel disparity correction in order to deal with the noise and bias at textured areas. It it important to note the subpixel correction does not only refine the final map, but most importantly, it helps the algorithm to propagate more correct messages, since $C_{d_p}(t_p^*)$ is always higher than $C_{d_p}(0)$ in (\ref{data_term1}).

Algorithm~\ref{our_algorithm} describes the steps of the process. To simplify its description, initial disparities $d_p\in\cal A\!\!\downarrow$ are augmented to meta-disparities $\mu_p$, i.e. $\mu_p = (d_p;0)$, which in turn initialize a set $\mathcal{M}$. We denote with $\mathcal{N} (\mu_p)= \{\mu_p^j\}_{j=1}^4$ the image-based neighbors of $\mu_p$, that is, $\mu_p^j=(d_{\hat p}; t_{\hat p})$ with $\hat{p}$ being any of the four immediate neighbors of $p$. Note that $\mu_p^j$ is not necessarily an element of $\cal M$.

The algorithm starts by sorting the elements of $\cal M$ based on their energy value, while it initializes to false the visit- and assignment-flag of all candidate meta-disparities. Next, it considers the lowest-energy $\mu_p$ with false visit-flag and switches this flag to true. Then, it assigns values at \emph{each} $\mu_p^j\in\cal N(\mu_p)$ with false assignment-flag based on the following minimization scheme
\begin{equation}\label{local_minimization}
    (d^*_{\hat p};t^*_{\hat p}) =
\underset{t_{\hat p},\,|d_{\hat p}-d^*_{p}|\leq r}{\arg\min}
 E(d_{\hat p};t_{\hat p}),
\end{equation}
where
\begin{equation}\label{detailed_local_energy}
    E(d_{\hat p};t_{\hat p}) =
    \eta_{\hat p}^S E_S(d_{\hat p};t_{\hat p})  + \eta_{\hat p}^A E_A(d_{\hat p})
\end{equation}
and $d^*_{p}$ is the optimum disparity of the parent node of $\hat{p}$. Note that (\ref{detailed_local_energy}) extends (\ref{local_energy}) by adding the subpixel disparity parameter into the stereo term and making the fusion pixel-dependent. In other words, what we do for each neighbor $\hat{p}$ with false assignment-flag is the following. For each candidate integer value $d_{\hat p}\in[d_p^*-r,d_p^*+r]$ the optimum $t_{\hat p}^*$ that minimizes the term $E_S(d_{\hat p};t_{\hat p})$ is obtained based on Proposition I and the local energy $E(d_p;t_p^*)$ is computed from (\ref{detailed_local_energy}). Among the $2r+1$ values, the disparity minimizer $d_{\hat p}^*$ is finally chosen and the corresponding subpixel correction is assigned, as shown in (\ref{local_minimization}). Recall that $r$ has a low value, in contrast to conventional stereo algorithms where it equals the whole disparity range. If $E(d_{\hat p}^*;t_{\hat p}^*)<T$, then the meta-disparity $(d_{\hat p}^*;t_{\hat p}^*)$ is pushed into $\mathcal{M}$ with respect to the sorting and its assignment-flag becomes true. The above process is repeated with unvisited meta-disparities until the cardinality of $\cal M$ remains fixed. The final set $\cal M$ corresponds to the final dense disparity map while a post-filling method can deal with missing disparities. It is important to note that the algorithm cannot get stuck in a loop since it propagates disparities in a tree structure while a true visit-flag can never be reset to false.

\begin{algorithm}[t!]\nonumber
\algsetup{linenosize=\scriptsize}
\caption{Stereo-Depth Fusion}
\begin{algorithmic}[1]
\REQUIRE Image-pair~$\mathcal{S}=\{I_L, I_R\}$, set~$\mathcal{A}\!\downarrow$, Threshold~$T$.
\STATE Compute the initial disparity map $D^0$ through $\mathcal{A}\!\downarrow$. %(by triangulation-based interpolation).
\label{s:initial_map}
\STATE Transform $\mathcal{A}\!\downarrow$ into a set $\mathcal{M}$ of meta-disparities with $t_p\!\!=\!0$.%\vskip -0.1cm
\STATE Sort $\cal M$'s elements based on their energy $E(\mu)$.\label{s:sorting}
\STATE Set both the visit and assignment flags $f_v(\mu)$, $f_a(\mu)$ to false, for all candidate meta-disparities, including $\mathcal{M}$.
\REPEAT
\STATE Consider $\mu_p$ with minimum energy and false $f_v(\mu_p)$% and set $f_v(\mu_p)=\text{true}$
\STATE Set $f_v(\mu_p)=\text{true}$
\FORALL{ $\mu_p^j \in \mathcal{N}(\mu_p)$ with $f_a(\mu_p^j)=\text{false}$}
\STATE  $\mu_p^{j*} = \arg\min E(\mu_p^j)~$ (Eq. \ref{local_minimization})
\IF{ $E(\mu_p^{j*})<T$}
\STATE Set $f_a(\mu_p^{j*})=\text{true}$
\STATE Push $\mu_p^{j*}$ in $\cal M$ w.r.t. sorting
\ENDIF
\ENDFOR
\UNTIL{$\text{card}(\cal M)$ is fixed}
\STATE Compute the dense disparity map $D$ from $\cal M$
\RETURN $D$.
\end{algorithmic}\label{our_algorithm}
\end{algorithm}\vskip -0.6cm


%The pseudocode of the proposed fusion algorithm is summarized in Algorithm 1.%\ref{our_algorithm}


==> tableHR_2_R2.tex <==
%\begin{figure*}[!b]
\begin{table*}[!h]
\centering
\caption{BMP for \emph{high-resolution} disparity maps of the Middlebury dataset with $\delta=2$.}
\footnotesize
\renewcommand{\arraystretch}{0.95}
\begin{tabular}{|p{1.30cm}|p{2.3cm}|c|c|c|c|c|c|c|c||c|}
  \hline
 &  &  Lampshade1 & Art & Monopoly & Rocks2 & Reindeer & Bowling2 & Baby1 & Moebius & Average\\
  \hline
\multirow{6}{*}{Stereo} &   
% GCS~\cite{Cech07}                                 & 16.2 & 12.1 & 44.9 & 1.9  & 7.3 & 16.6 & 10.9 & 14.0 & 15.4 \\
 GCS~[20]                                 & 16.2 & 12.1 & 44.9 & 1.9  & 7.3 & 16.6 & 10.9 & 14.0 & 15.4 \\
%&  ELAS~\cite{Geiger10}                               & 10.4 & 8.1 & 34.1 &  \underline{1.5} & \bf{3.6} & 10.6 & 6.5 & 11.3 & 10.7\\
&  ELAS~[21]                               & 10.4 & 8.1 & 34.1 &  \underline{1.5} & \bf{3.6} & 10.6 & 6.5 & 11.3 & 10.7\\
%&  GraphCuts~\cite{Kolmogorov01}                             & 22.9 & 17.9 & 56.1 & 5.4 & 18.1 & 31.0 & 9.3 & 13.6 & 21.7\\
&  GraphCuts~[52]                             & 22.9 & 17.9 & 56.1 & 5.4 & 18.1 & 31.0 & 9.3 & 13.6 & 21.7\\
%  \hline
%& CSBP~\cite{Yang2010ConstantSpaceBP}                 & 33.4 & 20.5 & 57.8 & 6.0 & 15.2 & 23.7 & 12.2 & 16.2 & 23.1\\
& CSBP~[28]                 & 33.4 & 20.5 & 57.8 & 6.0 & 15.2 & 23.7 & 12.2 & 16.2 & 23.1\\
% \hline
% & FastAgg~\cite{Rhemann2011fastCost}                  & 24.1 & \underline{8.0} & 41.6 & \bf{1.2} & \underline{4.8} & 13.0 & 8.8  & 12.9 & 14.3\\
 & FastAgg~[25]                  & 24.1 & \underline{8.0} & 41.6 & \bf{1.2} & \underline{4.8} & 13.0 & 8.8  & 12.9 & 14.3\\
% \hline
%& NonLocalAgg~\cite{Yang2012_nonLocaLCostAggregation} & 15.3 & 14.7 & 23.3 & 3.3 & 14.4 & 16.0 & 10.5 & 10.3 & 13.4\\
& NonLocalAgg~[27] & 15.3 & 14.7 & 23.3 & 3.3 & 14.4 & 16.0 & 10.5 & 10.3 & 13.4\\

%\hline
\hline
\multirow{2}{*}{Upsamping} & 
%Yang \emph{et al.}~\cite{Yang2007spatial}            & 16.4 & 22.7 & 16.9 & 17.2 & 18.5 & 15.7 & 11.9 & 19.5 & 17.3\\
Yang \emph{et al.}~[31]            & 16.4 & 22.7 & 16.9 & 17.2 & 18.5 & 15.7 & 11.9 & 19.5 & 17.3\\
%\hline& -
%& Kopf \emph{et al.}~\cite{Kopf2007jointBilateral}     & 9.2 & 12.9 & 9.6 & 8.9 & 10.6 & 10.4 & 8.7 & 10.4 & 10.1\\
& Kopf \emph{et al.}~[34]     & 9.2 & 12.9 & 9.6 & 8.9 & 10.6 & 10.4 & 8.7 & 10.4 & 10.1\\
\hline
 % EPC~\cite{Gandhi12}                               & 4.9 & 9.6 & \bf{5.7} & 2.3  & 4.7 & 3.7 & 2.9 & 5.6 & -\\ % with naive interpolation
\multirow{5}{*}{Fusion} &
%   EPC~\cite{Gandhi12}                               & 5.1 & 11.5 & 5.0 & 1.8  & 5.9 & 6.1 & 3.1 & 7.2 & 5.7\\%with bilateral upsampling& Vinnet's filling
   EPC~[15]                               & 5.1 & 11.5 & 5.0 & 1.8  & 5.9 & 6.1 & 3.1 & 7.2 & 5.7\\%with bilateral upsampling& Vinnet's filling

%\hline
%  F-MRF (GC)~\cite{Zhu08}                           & 12.9 & 12.8 & 16.5 & 1.4 & 10.9 & 19.2 & 6.2 & 7.8 & -\\ % with naive interpolation
% &  F-MRF (GC)~\cite{Zhu08}                           &  \bf{3.8} &  \bf{7.6} & 12.1 & 1.5 & 3.8 & 6.2 & \underline{2.4} & \bf{5.1} & 5.3\\  % with bilateral upsampling
 &  F-MRF (GC)~[12]                           &  \bf{3.8} &  \bf{7.6} & 12.1 & 1.5 & 3.8 & 6.2 & \underline{2.4} & \bf{5.1} & 5.3\\  % with bilateral upsampling
 & F-MRF (ICM)                                        & 6.3 & 14.1 & 27.8 & 6.2 & 5.8 & 8.0 & 5.2 & 9.2 & 10.3\\
%  \hline
%  F-ECC                                              & \bf{4.3} & \bf{6.8} & 6.6 & 1.9 & \bf{3.4} & 3.4 & 2.3 & \bf{5.2} & - \\  % with naive interpolation
 & F-ECC                                              & \underline{4.1} & 11.0 & \underline{3.8} & 1.6 & 5.3 & \underline{4.9} & \bf{2.3} & \underline{6.0} & \bf{4.8}\\  % with bilateral
%  \hline
%  F-EMCC                                            & 6.5 & 7.2 & 6.5 & 2.3 & 4.0 & 3.2 & 2.1 & 5.4 & -\\ %naive interpolation
&  F-EMCC                                             & 4.4 & 11.4 & \bf{3.6} & 1.9 & 5.1 & \bf{4.6} & 2.5 & 6.4 & \underline{5.0} \\ % bilateral upsampling

 % (Exp10 EMCC) & 7.4 & 5.2 & 7.1 & 10.2 & 1.3 & 3.6 & 2.9 & 1.5 & 8.0 \\

   \hline
 \multicolumn{11}{l}{  \scriptsize *see the manuscript for the references.}   
\end{tabular}
\label{table:HR_2}
\vskip -0.25cm
\end{table*}
%\end{figure*}

